On a Doubly Reduced Model for Dynamics of Heterogeneous Mixtures of Stiffened Gases, its Regularizations and their Implementations

We deal with the reduced four-equation model for the dynamics of heterogeneous compressible binary mixtures with the stiffened gas equations of state. We study its further reduced form, with the excluded volume concentrations, and with a quadratic equation for the common pressure of the components; this form can be called a quasi-homogeneous form. We prove new properties of the equation, derive simple formulas for the squared speed of sound and present an alternative proof for a formula that relates it to the squared Wood speed of sound; also, a short derivation of the pressure balance equation is given. For the first time, we introduce regularizations of the heterogeneous model (in the quasi-homogeneous form). Previously, regularizations of such type were developed only for the homogeneous mixtures of perfect polytropic gases, and it was unclear how to cover the case considered here. In the 1D case, based on these regularizations, we construct new explicit two-level in time and symmetric three-point in space finite-difference schemes without limiters, and provide numerical results for various flows with shock waves.

==> numerical <==
\section{Numerical experiments}

We present results of seven numerical experiments.

\begin{table}[h]
\caption{Stiffened gas parameters in 7 tests}
\label{tab:sgparams}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
%\textbf
{Substance}&$\gamma$
%, 1
&$c_v$, J/(kg K)&$p_\infty$, Pa&  $q$, J/kg \\[1mm]
\hline
\multicolumn{5}{|l|}{{1. Air-to-water shock tube problem}\cite{KLC14}}\\[1mm]
\hline
Air & 1.4 & 717.5&0&0\\[1mm]
\hline
Water & 2.8 & 1495&$8.5\cdot 10^8$&0\\[1mm]
\hline
\multicolumn{5}{|l|}{{2. Water-to-air shock tube problem}\cite{LF11}}\\[1mm]
\hline
Air & 1.4 & 720&0&0\\[1mm]
\hline
Water & 2.8 & 1495&$8.5\cdot 10^8$&0\\[1mm]
\hline
\multicolumn{5}{|l|}{{3. Shock tube test with a mixture containing mainly water vapor}\cite{CBS17IJNMF}}\\[1mm]
\multicolumn{5}{|l|}{{4. Shock tube test with a vanishing liquid phase}\cite{CBS17IJNMF}}\\[1mm]
\multicolumn{5}{|l|}{{5. Shock tube test with a mixture containing mainly liquid water}\cite{CBS17IJNMF}}\\[1mm]
\hline
Water vapor & 1.43 & 1040&0&$\hphantom{-}2030\cdot 10^3$\\[1mm]
\hline
Water & 2.35 & 1816 &$10^9$&$-1167\cdot 10^3$\\[1mm]
\hline
\multicolumn{5}{|l|}{{6. Dodecane vapor-to-liquid shock tube}\cite{YC13}}\\[1mm]
\hline
Vapor & 1.025 & 1956 &0&$-237 \cdot 10^3$\\[1mm]
\hline
Liquid & 2.35 & 1077&$4\cdot 10^8$&$-755\cdot 10^3$\\[1mm]
\hline
\multicolumn{5}{|l|}{{7. Carbon dioxide depressurization}\cite{LA12,ABR20}}\\[1mm]
\hline
Vapor & 1.06 & 2410 &$8.86\cdot 10^5$&$-3.01 \cdot 10^5$\\[1mm]
\hline
Liquid & 1.23 & 2440&$1.32\cdot 10^8$&$-6.23\cdot 10^5$\\[1mm]
\hline
\end{tabular}
\end{center}
\end{table}

%\smallskip\par \textbf{\ref{sect: numer experiments}
\subsection{Air-to-water shock tube problem}%Kitamura

A 10 m long tube is separated by left and right states, and the initial discontinuity is located in the middle of the tube. The left half is filled with air, and the right half is filled with water. The initial conditions are given in the table \ref{tab:initial}. The plots showing the total density of the mixture, along with the mass and volume fractions of the gas phase, pressure, velocity, and temperature of the mixture, are depicted in Fig. \ref{fig:kitamura} for QGD regularization. Note that we took quite standard values of the parameters, and quality of the solution is quite good. 

However, we may notice that we have a sort of parasitic invariability line around the rarefaction wave in air. The plot of the average velocity in \cite{KLC14} also had a segment that slightly differed from the invariability line in the solution, but that defect occurred around the shock in water. The additional invariability line from our experiment seems to be a consequence of our using a one-velocity and one-temperature model rather than the two-velocity and two-temperature one from \cite{KLC14}. 

However, in general, our numerical results correspond well to previously computed ones and the overall quality of the solution is at a good level.

\begin{figure*}[hbt!]
\center{\includegraphics[width=1\linewidth]{KitamuraAirToWater_Test}}
\caption{Numerical results for air-to-water shock tube problem 
(test \ref{sect: numer experiments}1) for $N= ?, 2000$, $a=0.3$ and $\beta=0.2$ (the QGD regularisation)}
\label{fig:kitamura}
\end{figure*}
%
%\begin{figure}[t]
%\center{\includegraphics[width=1\linewidth]{KitamuraAirToWater_Test_QHD}}
%\caption{Numerical results for air-to-water shock tube for $N= ?, 2000$, $a=0.6$ and $\beta=0.2$ (the QHD regularisation)}
%\label{fig:kitamuraqhd}
%\end{figure}

\subsection{Water-to-air shock tube problem}%LiFu

In this test, we again have a 10 m long tube separated into two halves. Now, however, the left half is filled with water, and the right half is filled with air. The initial conditions are given in the table \ref{tab:initial}.  The plots showing the total density of the mixture, along with the mass and volume fractions of the gas phase, pressure, velocity, and temperature of the mixture, are depicted in Fig. \ref{fig:lifu} for QGD regularization.

This is quite a unique case. Never before had we taken the value of $a$ exceeding 1! Although the computation doesn't fail if we take $0<a<1$ (that is the most often used interval, and before this experiment taking its values outside that interval was unheard of), the quality of the solutions turns out to be much worse. The greater we take the value of $a$, the more smoothed the solution becomes, as it can be seen, e.g. in the temperature plot.

The QHD regularization fails to compute this test.


\begin{figure*}[hbt!]
\center{\includegraphics[width=1\linewidth]{LiFuWaterToAir_Test}}
\caption{Numerical results for water-to-air shock tube (test \ref{sect: numer experiments}2) 
 for $N= ?, 2500$, $a=2$ and $\beta=0.1$ (the QGD regularisation)}
\label{fig:lifu}
\end{figure*}

\subsection{Shock tube test with a mixture containing mainly water vapor}%Chiapolino 6.1

In this test, we consider a 1 m long tube filled with a mixture that contains mainly water vapor: the initial vapor mass fraction is 0.8. All the initial conditions are given in table \ref{tab:initial}. The plots showing the total density of the mixture, along with the mass and volume fractions of the gas phase, pressure, velocity, and temperature of the mixture, are depicted in Fig. \ref{fig:chiapolino61qhd} for QHD regularization.

The results are in perfect agreement with \cite{CBS17IJNMF}.  

%\begin{figure}[h]
%\center{\includegraphics[width=1\linewidth]{Chiapolino61_Test}}
%\caption{Numerical results for shock tube with a mixture containing mainly water vapor for $N= ?, 500$, $a=0.2$ and $\beta=0.2$ (the QGD regularisation)}
%\label{fig:chiapolino61}
%\end{figure}
%
\begin{figure*}[hbt!]
\center{\includegraphics[width=1\linewidth]{Chiapolino61_Test_QHD}}
\caption{Numerical results for shock tube with a mixture containing mainly water vapor
(test \ref{sect: numer experiments}3) for $N= ?, 500$, $a=0.8$ and $\beta=0.2$ (the QHD regularisation)}
\label{fig:chiapolino61qhd}
\end{figure*}

\subsection{Shock tube test with a vanishing liquid phase}%Chiapolino 6.2

In this test, we consider a 1 m long tube filled with a mixture with a vanishing liquid phase: the initial liquid mass fraction is 0.01. All the initial conditions are given in table \ref{tab:initial}. The plots showing the total density of the mixture, along with the mass and volume fractions of the gas phase, pressure, velocity, and temperature of the mixture, are depicted in Fig. \ref{fig:chiapolino62} for QGD regularization.

\begin{figure*}[hbt!]
\center{\includegraphics[width=1\linewidth]{Chiapolino62_Test}}
\caption{Numerical results for shock tube with a vanishing liquid phase  (test \ref{sect: numer experiments}4) 
 for $N= ?, 500$, $a=0.2$ and $\beta=0.2$ (the QGD regularisation)}
\label{fig:chiapolino62}
\end{figure*}
%
%\begin{figure}[t]
%\center{\includegraphics[width=1\linewidth]{Chiapolino62_Test_QHD}}
%\caption{Numerical results for shock tube with a vanishing liquid phase for $N= ?, 500$, $a=0.8$ and $\beta=0.2$ (the QHD regularisation)}
%\label{fig:chiapolino62qhd}
%\end{figure}

\subsection{Shock tube test with a mixture containing mainly liquid water}%Chiapolino 6.3
In this test, we consider a 1 m long tube fiiled with a mixture that contains mainly liquid water: the initial vapor mass fraction is 0.2. All the initial conditions are given in table \ref{tab:initial}. The plots showing the total density of the mixture, along with the mass and volume fractions of the gas phase, pressure, velocity, and temperature of the mixture, are depicted in Fig. \ref{fig:chiapolino63qhd} for QHD regularization.
%\begin{figure}[h]
%\center{\includegraphics[width=1\linewidth]{Chiapolino63_Test}}
%\caption{Numerical results for shock tube with a mixture containing mainly liquid water for $N= ?, 500$, $a=0.2$ and $\beta=0.3$ (the QGD regularisation)}
%\label{fig:chiapolino63}
%\end{figure}
%
\begin{figure*}[hbt!]
\center{\includegraphics[width=1\linewidth]{Chiapolino63_Test_QHD}}
\caption{Numerical results for shock tube with a mixture containing mainly liquid water
(test \ref{sect: numer experiments}5) for $N= ?, 500$, $a=0.8$ and $\beta=0.3$ (the QHD regularisation)}
\label{fig:chiapolino63qhd}
\end{figure*}

\subsection{Dodecane vapor-to-liquid shock tube}
We consider the dodecane vapor-liquid shock tube solved by Yeom et al. \cite{YC13}: a 10 m long shock tube is filled with vapor dodecane under high pressure at the left, and with the liquid dodecane under atmospheric pressure at the right.
%The stiffened gas parameters are given in the Table \ref{tab:sgparams}.
The initial discontinuity is set at a distance of 3 m from the left, and the initial conditions are as follows
\[
(p_0,u_0,\theta_0)=
\begin{cases}
(10^{10}\text{ Pa}, 0 \text{ m/s}, 308.15\text{ K}), & -5 \leq x < -2\\
(10^5\text{ Pa}, 0 \text{ m/s}, 308.15\text{ K}), & -2 < x \leq 5
\end{cases}.
\]

The plots showing the total density of the mixture, along with the mass and volume fractions of the gas phase, pressure, velocity, and temperature of the mixture, are depicted in Fig. \ref{fig:yeomchang} for the QGD regularization and in Fig. \ref{fig:yeomchangqhd} for the QHD one.

The results obtained from the QHD regularization are slightly worse than in the QGD case, as we can notice a small nonphysical gap in the plots of temperature and gas volume fraction. Nonetheless, the overall quality of the solution under this regularization remains at an acceptable level.

The numerical profiles of the depicted functions correspond well to those presented in \cite{YC13}, although the wave in our model seems to propagate faster.

\begin{figure*}[hbt!]
\center{\includegraphics[width=1\linewidth]{YeomChang_Test}}
\caption{Numerical results for dodecane vapor-to-liquid shock tube (test \ref{sect: numer experiments}6) 
 for $N=2000$, $a=0.9$ and $\beta=0.1$ (the QGD regularisation)}
\label{fig:yeomchang}
\end{figure*}
%
%\begin{figure}[t]
%\center{\includegraphics[width=1\linewidth]{YeomChang_Test_QHD}}
%\caption{Numerical results for dodecane vapor-to-liquid shock tube for $N= ?, 2000$, $a=1.8$ and $\beta=0.1$ (the QHD regularisation)}
%\label{fig:yeomchangqhd}
%\end{figure}

\subsection{Carbon dioxide depressurization}
Here, we simulate depressurization of a 80-m long pipe that is filled with pure carbon dioxide. The pipe is filled with liquid carbon dioxide at the left, and with the gas carbon dioxide at the right. The stiffened gas parameters are given in Table \ref{tab:sgparams}.
The initial discontinuity is set at a distance of 50 m from the left, and the initial conditions are as follows:
\[
(p_0,u_0,\theta_0)=
\begin{cases}
(6\cdot10^{6}\text{ Pa}, 0 \text{ m/s}, 283.13\text{ K}), & -40 \leq x < 10\\
(10^6\text{ Pa}, 0 \text{ m/s}, 283.13\text{ K}), & 10 < x \leq 40
\end{cases}.
\]

The plots showing the total density of the mixture, along with the mass and volume fractions of the gas phase, pressure, velocity, and temperature of the mixture, are depicted in Fig. \ref{fig:abgrall} for the QGD regularization and in Fig. \ref{fig:abgrallqhd} for the QHD one.

In this test, we had to take $a_{Pr}=0.1$ (i.e., increase heat conductivity). 
For QGD regularization, the quality of the solution is good and corresponds well to both the results of \cite{LA12} and \cite{ABR20}. However, the QHD regularization behaves worse in this case. 
If we only double the value of $\alpha$, the computations fail. 
Thus, we decided to halve the $\beta$ parameter. 
After that, the computation completed successfully. However, the quality of the velocity plot worsened: we can see a strange slope on the borders of the phases.
Also, the gap on the temperature plot is more noticeable than on the corresponding plot for the QGD case.

\begin{figure*}[hbt!]
\center{\includegraphics[width=1\linewidth]{AbgrallBacigaluppiRe_Test}}
\caption{Numerical results for carbon dioxide depressurization (test \ref{sect: numer experiments}7) 
 for $N= ?, 4000$, $a=0.8$ and $\beta=0.1$ (the QGD regularisation)}
\label{fig:abgrall}
\end{figure*}

\begin{acknowledgments}
This study was supported by the Russian Science Foundation, grant no. 22-11-00126
(A.~Zlotnik, Sections II and III)
%\ref{sect: Quasi-Homogeneous Mixt} and \ref{sect: regularized system}) 
and
by the Moscow Center of Fundamental and Applied Mathematics Agreement with the Ministry of Science and Higher Education of the Russian Federation, grant no.~075-15-2022-283
(the both authors, Sections IV and V).
\end{acknowledgments}

\section*{Data Availability Statement}

The data that support the findings of this study are available from the corresponding author upon reasonable request.
